Bandit Learning to Rank with Position-Based Click Models: Personalized and Equal Treatments

Online learning to rank (ONL2R) is a foundational problem for recommender systems and has received increasing attention in recent years. Among the existing approaches for ONL2R, a natural modeling architecture is the multi-armed bandit framework coupled with the position-based click model. However, developing efficient online learning policies for MAB-based ONL2R with position-based click models is highly challenging due to the combinatorial nature of the problem, and partial observability in the position-based click model. To date, results in MAB-based ONL2R with position-based click models remain rather limited, which motivates us to fill this gap in this work. Our main contributions in this work are threefold: i) We propose the first general MAB framework that captures all key ingredients of ONL2R with position-based click models. Our model considers personalized and equal treatments in ONL2R ranking recommendations, both of which are widely used in practice; ii) Based on the above analytical framework, we develop two unified greed- and UCB-based policies called GreedyRank and UCBRank, each of which can be applied to personalized and equal ranking treatments; and iii) We show that both GreedyRank and UCBRank enjoy $O(\sqrt{t}\ln t)$ and $O(\sqrt{t\ln t})$ anytime sublinear regret for personalized and equal treatment, respectively. For the fundamentally hard equal ranking treatment, we identify classes of collective utility functions and their associated sufficient conditions under which $O(\sqrt{t}\ln t)$ and $O(\sqrt{t\ln t})$ anytime sublinear regrets are still achievable for GreedyRank and UCBRank, respectively. Our numerical experiments also verify our theoretical results and demonstrate the efficiency of GreedyRank and UCBRank in seeking the optimal action under various problem settings.

==> Sec1_Introduction/Introduction_Tianchen.tex <==
% !TEX root = ../paper.tex

\section{Introduction} \label{sec:introduction}

Learning to rank is a foundational and key problem in many recommender systems \cite{sorokina2016amazon}.
For example, Google, the most dominant search engine company, announced a revenue of \$40,689 million on search advertising for the second quarter of 2022~\cite{Document21:online}.
Most of the existing literature focuses on offline learning to rank, which studies the relevance of query-url pair based on training pairs, then applies the learned model on relevance prediction and ranking.
Such offline method generates static ranking models while facing the situation where new customer data keeps coming, and the quality of the obtained models highly depends on the quality of training pairs.
Therefore, in recent years, more works turn to study online learning to rank \cite{agichtein2006improving}.
Among the proposed frameworks, multi-armed bandit (MAB) is shown to be efficient for online learning to rank \cite{radlinski2008learning,lagree2016multiple,zoghi2017online,lattimore2018toprank}, which formulates the sequential interaction of platform and customers.
In MAB-based online learning to rank models, at each round, the learner makes decisions on item ranking and observes the reward corresponding to the ranking decision, where the reward is typically interpreted as user behavior such as clicks.

This paper focuses on ranking with position-based model \cite{chuklin2015click}, where each ranking position is attributed with a preference probability indicating it's visibility.
Position-based click model has been widely used to formulate user behavior \cite{richardson2007predicting, lagree2016multiple}, as many investigations show that user actions are highly relevant to website layout or ranking positions.
One example is Google Golden Triangle \cite{hotchkiss2005eye}, which shows that in sponsered search, if a listing is not displayed in some particular area of the web layout, then the odds of being seen by a searcher are dramatically reduced.
In e-commerce platforms, normalized discounted cumulative gain (NDCG) is a commonly used metric to measure the quality of item rankings.
NDCG applies a discounted weight on each ranking position, that decreases logarithmically with backwards ranked positions.
The position-based model shares a very close idea with the definition of NDCG, and thus is a suitable model for ranking problems in e-commerces.
We remark two aspects on position-based model: (i) the position preferences can usually be statistically computed by historical user actions, however, in the early stage of online ranking systems without enough historical data, the position preferences also require estimation from sequential user actions, and may sacrifice some ranking quality; (ii) demographic studies \cite{hotchkiss2005eye} show that there exist many different user action patterns that are related to user's gender, education, age, etc, such as the quick click, the linear scan, the deliberate scan, the pick up search, etc, so the same position can have different preference rates over different groups of people, which is overlooked by most of the related literature.
% However, most existing literature assumes known and homogeneous position preferences \cite{lagree2016multiple}, which is unrealistic in practice.

The setting of different user types has been rarely considered in online ranking literature.
One crucial reason is that, bandit based online ranking models typically generate arm rankings by computing an optimistic index for each arm and ranking all the indices.
In the simpler setting of one user type, arm rankings can be obtained by simply decreasingly ranking all the indices, while in the setting of multiple user types, each arm has a vector of optimistic indices, and obtaining arm rankings usually becomes an integer convex optimization that solved in exponentially increasing time as the system size grows.
This optimization needs to be carried out every time a new ranking is requested.
Such a problem size is a bottleneck of applying theoretical policies to practice, and still needs future research \cite{biega2018equity}.
This paper takes an early step on the setting of multiple user types.
With different user behavior among different user types, two ranking strategies are considered in the model: personalization and equal treatment, both are widely applied in real-world.
Personalization strategies recommend group-wise optimal rankings and allows different rankings among user groups, which maximize user experience.
However, for user groups denoted by sensitive attributes, service providers are legally required to avoid differentiated treatment, i.e., they should treat all sensitive groups equally, by recommending similar content to all groups of people. Therefore, recommending one ranking to all users is a requirement for fair treatment, and social welfare is a well-known metric for resource allocation with fairness consideration \cite{midgley1997social}.

The contributions of this paper are highlighted as follows: (a) we study bandit online ranking with multiple user types where user feedback is partial observable and is generated from two unkown parameters: position preferences and arm means, then we propose policies that provide rankings in two strategies: personalization and equal treatment.
Theoretical results show that all the proposed policies achieves sub-linear regret over time.
(b) We discuss the impact of system size on the time complexity of searching rankings. The proposed equal treatment ranking policies allow approximation algorithms, which reduce the time complexity for searching rankings.
Theoretical results show that with the approximation algorithms in some accuracy, the proposed policies can still reach sub-linear regret.
(c) we show the validity and efficiency of our policies by conducting experiments on synthetic datasets and real-world datasets.







% Learning to rank is a foundational and key problem in many recommender systems, such as search engines, video streaming services, and online shopping in e-commerce~\cite{sorokina2016amazon}.
% Solving a learning to rank problem amounts to understanding and predicting users' browsing and clicking behaviors, so that the system can provide an optimal ranking accordingly to maximize certain rewards or utilities.
% For example, Google, the most dominant search engine company, announced a revenue of \$40,689 million on search advertising for the second quarter of 2022~\cite{Document21:online}.
% Meanwhile, the quality of learning to rank could also have a huge impact on users' browsing and clicking behaviors.
% Studies showed that, in sponsored search (i.e., content providers pay search engines for directing traffic to their websites), the probability of a user clicking on an ad changes dramatically with the ad's display position~\cite{hotchkiss2005eye}.
% In the literature, learning to rank has been relatively well studied in the supervised setting, where an offline dataset provides all the necessary relevance factors needed for ranking.
% However, in contrast to the offline counterpart, online learning to rank remains under-explored in the research community and results are rather limited so far (see Section~\ref{sec:related} for detailed discussions).
% Meanwhile, as studies showed that incorporating real-time and historic user behavior data can significantly improve the ranking quality of top results in real-world recommender systems~\cite{agichtein2006improving}, online learning to rank has received increasing attention in recent years.

% Generally speaking, online learning to rank problems for recommender systems can be viewed as understanding and predicting users' click models~\cite{chuklin2015click} through {\em bandit feedback} (i.e., data are collected in real-time through action-reward interactions rather than preexisting).
% Based on such bandit feedback and following an online learning policy, the system iteratively adjusts the ranking of items to the next arriving user to maximize its long-term accumulative reward (e.g., user satisfaction).
% Some attempts on online learning to rank focused on learning the cascade model \cite{kempe2008cascade, kveton2015cascading} (i.e., assuming that users sequentially browse through a ranking, then click an item which they find attractive and stop browsing).
% Another click model, the position-based model~\cite{richardson2007predicting, lagree2016multiple} (i.e., assuming that the probability of each item being clicked depends on its relevance and ranked position) also attracts wide attention and is adopted in this paper due to its generality.
% Moreover, due to the use of bandit feedback, many online learning to rank problems are naturally formulated based on the multi-armed bandit framework (MAB) (see, e.g., \cite{radlinski2008learning,lagree2016multiple,zoghi2017online,lattimore2018toprank} and Section~\ref{sec:related} for detailed discussions). 


% %Online ranking methods have been proposed based on different click models to maximize the user satisfaction.
% However, despite the recent advances mentioned above,
% %to the best of our knowledge, 
% all existing MAB-based online ranking policies have overlooked one important performance metric -- {\em fairness}.
% %implicitly assume that user behavior is consistent over time.
% %In other words, each ranking item has equivalent attractiveness to any users.
% %However, such assumption is too strong in real world.
% For example, males and females are likely to have different preferences when choosing a book from a given recommended ranking list.
% An MAB policy for online ranking that maximizes the satisfaction of one gender will lead to low satisfaction to the other and result in fairness issues.
% \textcolor{blue}{On the other hand, in many situations service providers are legally required to avoid differentiated treatment, i.e., they should treat all sensitive groups equally, by recommending similar content to people from different sensitive groups. Therefore, recommending one ranking to all users is a requirement for fair treatment, and social welfare is a well-known metric for resource allocation with fairness consideration.}
% % Therefore, for online recommender systems that serve a large variety of users, it is important to design MAB-based ranking policies with appropriate fairness considerations over all potential user types.
% The lack of studies on MAB-based ranking policy designs for maximizing social welfare in terms of fairness motivates us to fill this important gap in this paper.
% Moreover, different from all existing fairness-aware MAB methods (see Section~\ref{sec:related}), our focus is on generic fairness-based social welfare maximization for the {\em position-based click model}, which is the most relevant for solving online learning to rank problems.

% However, developing MAB-based online ranking policies for the position-based click model is highly non-trivial due to the following technical challenges:
% %Considering fair objectives in position-based ranking problems brings out a series of challenges that has never been considered previously in related literature. Some key challenges are listed as follows:
% \begin{list}{\labelitemi}{\leftmargin=1.5em \itemindent=-0.0em \itemsep=-.1em}
% \vspace{-.1in}

% \item[1)] MAB-based online ranking policies with the position-based click model is inherently a {\em combinatorial} MAB problem, with exponentially large search spaces of all potential ranking and click position permutations. 
% As shown later, one often needs to address NP-hard challenges arising from MAB policy design and regret analysis.
% As a result, care must be taken to address the trade-offs between regret performance and complexity.

% \item[2)] The MAB policy design for fairness maximization with the position-based click model needs to {\em simultaneously} learn multiple system parameters with unknown distributions, including the arrival rates of different user groups, arms' mean attractiveness, and users' observation and selection probabilities of different arms.
% Thus, the number of parameters to learn is far more than that of conventional MAB problems.
% Exacerbating the problem is the fact that many fairness utility functions for social welfare are {\em nonlinear}, which prevents the use of simple sorting as a component in MAB policy design.
% \end{list}

% \vspace{-.1in}
% In this paper, we overcome the above challenges by proposing two online ranking MAB policies with sublinear regrets under various approximation conditions.
% Our main contributions are summarized as follows:
% \begin{list}{\labelitemi}{\leftmargin=1em \itemindent=-0.0em \itemsep=-.1em}
% \vspace{-.1in}
% \item We first formulate a fairness-based utility maximization problem for social welfare with the position-based click model. 
% Our formulation allows general fairness utility functions corresponding to a large number of social welfare criteria (e.g., utilitarian and Nash social welfare).

% \item To solve the fairness utility maximization problem, we propose two online learning to rank MAB policies, namely GreedyRank and UCBRank. 
% Both policies are efficient in maximizing fairness utility for social welfare in the presence of uncertainty and complex user behavior. 
% We show that the expected cumulative regrets of the proposed policies grow sublinearly over time, which even hold under appropriate approximation conditions when the underlying problem may be NP-hard.

% \item We conduct numerical experiments on various fairness utilities for social welfare and demonstrate the efficiency of the proposed MAB policies. 
% Our experiment results also illustrate the impacts of different fairness criteria on regret regret performances.
% \end{list}
